FLuRKA: Fast and accurate unified Low-Rank & Kernel Attention

Many efficient $\textit{approximate}$ self-attention techniques have become prevalent since the inception of the transformer architecture. Two popular classes of these techniques are low-rank and kernel methods. Each of these methods has its strengths. We observe these strengths synergistically complement each other and exploit them to fuse low-rank and kernel methods, producing a new class of transformers: FLuRKA ($\textbf{F}$ast $\textbf{L}$ow-$\textbf{R}$ank & $\textbf{K}$ernel$ \textbf{A}$ttention). FLuRKA are highly $\textit{training-efficient}$ with faster model speeds $\textit{and}$ similar model qualities compared to constituent low-rank and kernel methods. We theoretically and empirically evaluate the speed and quality of FLuRKA. Our model speed analysis posits a variety of parameter configurations where FLuRKA exhibit speedups over low-rank and kernel approximations and our model quality analysis bounds the error of FLuRKA with respect to full-attention. Empirically, we instantiate three FLuRKA variants which experience speedups of up to 3.3x and 1.7x over low-rank and kernel methods respectively. This translates to speedups of up to 20x over models with flash-attention. Across a diverse set of tasks spanning language modeling, language understanding, long sequence modeling, machine translation, and image classification, FLuRKA achieve comparable accuracy with underlying low-rank and kernel approximations, occasionally surpassing both.

==> analysis.tex <==
We theoretically analyze different arrangements where \name{} incur fewer FLOPs compared to low-rank and kernel methods. We present a range of arrangements that demonstrates high efficiency when scaling across the dimensions: sequence length, hidden dimension, and downsampling factor, improving model expressiveness while retaining efficiency.
%Empirically, as demonstrated in Section~\ref{}, these configurations lead to speedups of up to 3.3x and 1.7x over low-rank and kernel techniques, respectively. 
Additionally, we theoretically show that \name{} experience tight approximation error with respect to full-attention. Our analysis is general, bounding the error of a \textit{generic} \name{} under reasonable assumptions.  

\textbf{Efficiency Analysis} We first analyze where \name{} incurs fewer FLOPs compared to low-rank methods, kernel methods as well as both \textit{at the same time}. 
%We make theoretical claims delineating the precise arrangement of parameters that leads to these performance benefits. Specifically:
\begin{claim}
    For sequence length: $N$, hidden dimension: $d_m$, downsampling factor: $d_k$, head hidden dimension $d_h$, number of heads $H$, when: $$N > d_k(H+2) > d_m > d_k > d_h$$ \name{} incur lower FLOPs against both kernel and low-rank methods.
    \label{claim:one}
\end{claim}
\begin{claim}
    For sequence length: $N$, downsampling factor: $d_k$, head hidden dimension: $d_h$ when: $$N-1 > d_k> d_h $$ \name{} incur lower FLOPs against low-rank methods. 
    \label{claim:two}
\end{claim}
\begin{claim}
    For sequence length: $N$, hidden dimension: $d_m$, downsampling factor: $d_k$, number of heads: $H$, when: $$N > d_k(H+2), d_m > d_k$$ \name{} incur lower FLOPs against kernel methods.
    \label{claim:three}
\end{claim}
Each of the above claims delineates a \textit{regime} where \name{} exhibit competitive performance over low-rank and kernel techniques. Moreover, each bound is tight, requiring sequence lengths larger than 1k to imply speedups. See Appendix for proofs of these claims. 
